The Companion Model -- a Canonical Model in Graph Signal Processing

This paper introduces a $\textit{canonical}$ graph signal model defined by a $\textit{canonical}$ graph and a $\textit{canonical}$ shift, the $\textit{companion}$ graph and the $\textit{companion}$ shift. These are canonical because, under standard conditions, we show that any graph signal processing (GSP) model can be transformed into the canonical model. The transform that obtains this is the graph $z$-transform ($\textrm{G$z$T}$) that we introduce. The GSP canonical model comes closest to the discrete signal processing (DSP) time signal models: the structure of the companion shift decomposes into a line shift and a signal continuation just like the DSP shift and the GSP canonical graph is a directed line graph with a terminal condition reflecting the signal continuation condition. We further show that, surprisingly, in the canonical model, convolution of graph signals is fast convolution by the DSP FFT.

==> macrosmanuela.tex <==
\newenvironment{s_itemize}{\begin{list}{$\bullet$}
{\setlength{\rightmargin}{\leftmargin}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0em}
\setlength{\parsep}{0em}}}{\end{list}}

\newenvironment{s_itemize_2}{\begin{list}{$-$}
{\setlength{\rightmargin}{0em}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0em}
\setlength{\parsep}{0em}}}{\end{list}}

\newenvironment{s_itemize_3}{\begin{list}{$-$}
{\setlength{\rightmargin}{0em}\setlength{\leftmargin}{0em}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0em}
\setlength{\parsep}{0em}}}{\end{list}}

\newenvironment{noinds_itemize}{\begin{list}{$\bullet$}
{\setlength{\rightmargin}{0em}
\setlength{\leftmargin}{1.2em}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0em}
\setlength{\parsep}{0em}}}{\end{list}}

\newenvironment{small_ind_itemize}{\begin{list}{$\bullet$}
{\setlength{\rightmargin}{1em}
\setlength{\leftmargin}{2em}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0em}
\setlength{\parsep}{0em}}}{\end{list}}

\def\descriptionnobflabel#1{\hspace\labelsep #1}
\def\descriptionnobf{\list{}{\labelwidth\z@ \itemindent-\leftmargin
 \let\makelabel\descriptionnobflabel}}
\let\enddescriptionnobf\endlist

\def\s_descriptionlabel#1{\hspace\labelsep \bf #1}
\newenvironment{s_description}{\begin{list}{1}
{\setlength{\rightmargin}{\leftmargin}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0em}
\setlength{\parsep}{0em}
\renewcommand{\makelabel}{\s_descriptionlabel}}}{\end{list}}

\def\s_descriptionlabel#1{\hspace\labelsep \bf #1}
\newenvironment{s_description_nomargin}{\begin{list}{1}
{\setlength{\rightmargin}{0em}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0em}
\setlength{\parsep}{0em}
\renewcommand{\makelabel}{\s_descriptionlabel}}}{\end{list}}


\newenvironment{s_description_nobf}{\begin{list}{1}
{\setlength{\rightmargin}{\leftmargin}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0em}
\setlength{\itemindent}{1em}
\setlength{\parsep}{0em}}}{\end{list}}

\newcommand{\bind}[1]{\hspace*{#1}\begin{minipage}[t]{7in}\begin{itemize}}
\newcommand{\eind}{\end{itemize}\end{minipage}\\}
\newenvironment{inditem}
{\hspace*{1cm}\begin{minipage}[t]{6in}\begin{itemize}}
{\end{itemize}\end{minipage}}

\newenvironment{inditemize}{\begin{list}{$\bullet$}
{\setlength{\rightmargin}{\leftmargin}
\setlength{\itemsep}{\itemsep}
\setlength{\topsep}{\topsep}
\setlength{\itemindent}{1em}
\setlength{\parsep}{\parsep}}}{\end{list}}

\newenvironment{dinditemize}{\begin{list}{$-$}
{\setlength{\rightmargin}{\leftmargin}
\setlength{\itemsep}{\itemsep}
\setlength{\topsep}{\topsep}
\setlength{\itemindent}{1em}
\setlength{\parsep}{\parsep}}}{\end{list}}

\newenvironment{nobulletinditemize}{\begin{list}{}
{\setlength{\rightmargin}{\leftmargin}
\setlength{\itemsep}{\itemsep}
\setlength{\topsep}{\topsep}
\setlength{\itemindent}{0em}
\setlength{\parsep}{\parsep}}}{\end{list}}

\newenvironment{nobullets_itemize}{\begin{list}{}
{\setlength{\rightmargin}{0em}
\setlength{\leftmargin}{0.7em}
\setlength{\itemsep}{0.5em}
\setlength{\topsep}{0.5em}
\setlength{\parsep}{\parsep}}}{\end{list}}


\newenvironment{s_itemize_sp}{\begin{list}{$\bullet$}
{\setlength{\rightmargin}{0em}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0em}
\setlength{\parsep}{0em}}}{\end{list}}

\newcounter{ctr}
\newenvironment{indenumerate}{\begin{list}{\thectr.}
{\usecounter{ctr}
\setlength{\rightmargin}{\leftmargin}
\setlength{\itemsep}{\itemsep}
\setlength{\topsep}{\topsep}
\setlength{\itemindent}{1em}
\setlength{\parsep}{\parsep}}}{\end{list}}

%% just tight
\newenvironment{t_enumerate}{\begin{list}{\thectr.}
{\usecounter{ctr}
\setlength{\rightmargin}{\leftmargin}
\setlength{\itemsep}{0em}
\setlength{\topsep}{\topsep}
\setlength{\itemindent}{\itemindent}
\setlength{\parsep}{\parsep}}}{\end{list}}

\newenvironment{s_enumerate_noindent}{\begin{list}{\thectr.}
{\usecounter{ctr}
\setlength{\rightmargin}{0cm}
\setlength{\leftmargin}{0.5cm}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0em}
\setlength{\itemindent}{0cm}
\setlength{\parsep}{0em}}}{\end{list}}

\newenvironment{s_enumerate_noindent1}{\begin{list}{\thectr.}
{\usecounter{ctr}
\setlength{\rightmargin}{0cm}
\setlength{\leftmargin}{0em}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0em}
\setlength{\itemindent}{1.25em}
\setlength{\parsep}{0em}}}{\end{list}}


\newenvironment{s_enumerate}{\begin{list}{\thectr.}
{\usecounter{ctr}
\setlength{\rightmargin}{0.3cm}
\setlength{\leftmargin}{0.3cm}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0em}
\setlength{\itemindent}{0.5cm}
\setlength{\parsep}{0em}}}{\end{list}}

\newenvironment{s_enumerate_ltr}{\begin{list}{\theenumii.}
{\usecounter{enumii}
\setlength{\rightmargin}{0.3cm}
\setlength{\leftmargin}{0.3cm}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0em}
\setlength{\itemindent}{0.4cm}
\setlength{\parsep}{0em}}}{\end{list}}


\def\nolineslidehead#1{\newpage\begin{center}\begin{tabular*}{469pt}[t]{c}
\Huge{\parbox[c]{457pt}{\bf #1}} \\ \vspace{7pt} \\
\end{tabular*}\end{center}\yskip}

\def\centerslidehead#1{\newpage\begin{center}{\Huge{\bf #1}}\end{center}\yskip}

\def\slide#1{
 \newpage
 \begin{center}
 {\LARGE\bf {#1}}
 \end{center}
 \vspace{0in}}

\def\black{\special{ps:0 0 0 setrgbcolor}}

\def\red{\special{ps:0.8666 0.03137 0.02352 setrgbcolor}}
    %\newcommand{\red}{\special{ps:1 0 0 setrgbcolor}}

\def\blue{\special{ps:0.00784 0.67059 0.91764 setrgbcolor}}
    %\newcommand{\blue}{\special{ps:0 0 1 setrgbcolor}}

\def\green{\special{ps:0 0.68235 0 setrgbcolor}}
    %\newcommand{\green}{\special{ps:0 1 0 setrgbcolor}}

\def\royalblue{\special{ps:0 0.2 0.91764 setrgbcolor}}
\def\brickred{\special{ps:0.644541 0.164065 0.164065 setrgbcolor}}
\def\yellow{\special{ps:1 1 0 setrgbcolor}}
\def\brown{\special{ps:0.6 0.4 0.4 setrgbcolor}}
\def\orange{\special{ps:1 0.647059 0 setrgbcolor}}
\def\indigo{\special{ps:0.746105 0 0.996109 setrgbcolor}}
\def\violet{\special{ps:0.308598 0.183597 0.308598 setrgbcolor}}
\def\white{\special{ps:1 1 1 setrgbcolor}}
\def\lightgrey{\special{ps:0.762951 0.762951 0.762951 setrgbcolor}}
\def\darkgrey{\special{ps:0.503548 0.503548 0.503548 setrgbcolor}}
\def\pink{\special{ps:1 0.6 0.6 setrgbcolor}}


\newenvironment{tightlist}{
    \begin{itemize}
    \itemsep=0pt \parskip=0pt \parsep=0pt }{
    \end{itemize}
}

\newcommand{\boxedfigure}[2]{\vspace{1ex}
                             \fbox{\begin{minipage}[t]{#1} #2 \end{minipage}}
                             \vspace{1ex}}

\newenvironment{s_itemize-2}{\begin{list}{$\rhd$}
{\setlength{\rightmargin}{0em}
\setlength{\itemsep}{0em}
\setlength{\topsep}{0.25cm}
\setlength{\parsep}{0em}}}{\end{list}}

%% Big separation between items
\newenvironment{itemize-1}{\begin{list}{$\bullet$}
{\setlength{\rightmargin}{0em}
\setlength{\itemsep}{0.5cm}
\setlength{\topsep}{0.25cm}
\setlength{\parsep}{0em}}}{\end{list}}

\newenvironment{itemize-2}{\begin{list}{$\rhd$}
{\setlength{\rightmargin}{0em}
\setlength{\itemsep}{0.25cm}
\setlength{\topsep}{0.25cm}
\setlength{\parsep}{0em}}}{\end{list}}

\def\topslidehead#1{\newpage\begin{center}\vspace*{-3cm}\begin{tabular*}{469pt}[t]{c}
\Huge{\parbox[c]{457pt}{\bf #1}} \\ \vspace{7pt} \\
\end{tabular*}\end{center}\yskip}


% for smaller vspace in item list
\newenvironment{bullist}
    {\begin{list}{$\bullet$}
        {\parsep 0pt \itemsep 0pt \setlength{\rightmargin}{\leftmargin}}}%
    {\end{list}}
\newenvironment{dashlist}
    {\begin{list}{$-$}
        {\parsep 0pt \itemsep 0pt \setlength{\rightmargin}{\leftmargin}}}%
    {\end{list}}



\newenvironment{itemize-3}{\begin{list}{-}
{\setlength{\rightmargin}{0em}
\setlength{\itemsep}{0.25cm}
\setlength{\topsep}{0.25cm}
\setlength{\parsep}{0em}}}{\end{list}}

\newenvironment{itemize-4}{\begin{list}{\ }
{\setlength{\rightmargin}{0em}
\setlength{\itemsep}{0.25cm}
\setlength{\topsep}{0.25cm}
\setlength{\parsep}{0em}}}{\end{list}}


\newenvironment{short-itemize}{\begin{list}{$\bullet$}
{\setlength{\rightmargin}{0em}
\setlength{\itemsep}{0.10cm}
\setlength{\topsep}{0.10cm}
\setlength{\parsep}{0em}}}{\end{list}}




%kludge if you don't have the font on hand:
% New & Improved number sets (Andrej).
\font\sf=cmss10
\newcommand{\Nats}{{\hbox{\sf I\kern-.13em\hbox{N}}}}   % Natural numbers
\newcommand{\Reals}{{\hbox{\sf I\kern-.14em\hbox{R}}}}  % Real numbers
\newcommand{\Ints}{{\hbox{\sf Z\kern-.43emZ}}}          % Integers
\newcommand{\CC}{{\hbox{\sf C\kern -.48emC}}}           % Complex numbers
\newcommand{\QQ}{{\hbox{\sf C\kern -.48emQ}}}           % Rational numbers

\newcommand{\lNats}{{\hbox{\sf {\large I\kern-.13em\hbox{N}}}}}   %Natural numbers
\newcommand{\lReals}{{\hbox{\sf {\large I\kern-.14em\hbox{R}}}}}  %Real numbers
\newcommand{\lInts}{{\hbox{\sf {\large Z\kern-.43emZ}}}}          %Integers
\newcommand{\lCC}{{\hbox{\sf {\large C\kern -.48emC}}}}           %Complex numbers
\newcommand{\lQQ}{{\hbox{\sf {\large C\kern -.48emQ}}}}           %Rational numbers


